Curvy: A Parametric Cross-section based Surface Reconstruction

In this work, we present a novel approach for reconstructing shape point clouds using planar sparse cross-sections with the help of generative modeling. We present unique challenges pertaining to the representation and reconstruction in this problem setting. Most methods in the classical literature lack the ability to generalize based on object class and employ complex mathematical machinery to reconstruct reliable surfaces. We present a simple learnable approach to generate a large number of points from a small number of input cross-sections over a large dataset. We use a compact parametric polyline representation using adaptive splitting to represent the cross-sections and perform learning using a Graph Neural Network to reconstruct the underlying shape in an adaptive manner reducing the dependence on the number of cross-sections provided.

==> images/parametric_graph.tex <==
%% Creator: Inkscape inkscape 0.91, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'parametric_graph.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{574.18528bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \scalebox{1}{
  \begin{picture}(1,0.4)%
    %\put(0,0){\includegraphics[width=\unitlength]{images/parametric_graph.pdf}}%
    \put(0.18,0.32){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$f_j(t)$}}}%
    \put(0,0){\includegraphics[width=\unitlength]{images/parametric_graph.pdf}}%
    \put(0.65,0.4){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$[\theta_{0,j}, \cdots, \theta_{p,j}]$}}}%
    \put(0.0, 0.01){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\emph{Piecewise curve}}}}%
    \put(0.69,0.01){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{\emph{Piece-level graph}}}}%
  \end{picture}
  }
\endgroup%


==> sample-base <==

% Journals

% First the Full Name is given, then the abbreviation used in the AMS Math
% Reviews, with an indication if it could not be found there.
% Note the 2nd overwrites the 1st, so swap them if you want the full name.

 %{AMS}
@article{sawdayee2022orex,
  title={OReX: Object Reconstruction from Planner Cross-sections Using Neural Fields},
  author={Sawdayee, Haim and Vaxman, Amir and Bermano, Amit H},
  journal={arXiv preprint arXiv:2211.12886},
  year={2022}
}
 
@inproceedings{gadelha2018multiresolution,
  title={Multiresolution tree networks for {3D} point cloud processing},
  author={Gadelha, Matheus and Wang, Rui and Maji, Subhransu},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={103--118},
  year={2018}
}

@inproceedings{achlioptas2018learning,
  title={Learning representations and generative models for {3D} point clouds},
  author={Achlioptas, Panos and Diamanti, Olga and Mitliagkas, Ioannis and Guibas, Leonidas},
  booktitle={International conference on machine learning},
  pages={40--49},
  year={2018},
  organization={PMLR}
}

@String{cgforum = "Computer Graphics Forum"}
@String{tog = "ACM TOG"}

@article{Buhmann:1998:DCQ,
	AUTHOR = {J. M. Buhmann and D. W. Fellner and M. Held and J.
		Ketterer and J. Puzicha},
	TITLE = {Dithered Color Quantization},
	JOURNAL = cgforum,
	EDITOR = {N. Ferreira and M. G\"{o}bel},
	VOLUME = {17},	NUMBER = {3},
	MONTH = Sep,	YEAR = {1998},	PAGES = {C219-C231},
	DOI = {10.1111/1467-8659.00269},
  NOTE = {(Proc. Eurographics'98)
	       \httpsAddr{//diglib.eg.org/handle/10.2312/8491}} }

@ARTICLE{Fellner-Helmberg93,
	AUTHOR = {Fellner, Dieter W. and Helmberg, Christoph},
	TITLE = {Robust Rendering of General Ellipses and Elliptical Arcs},
	JOURNAL = tog,
	VOLUME = {12},	NUMBER = {3},
	MONTH = Jul,	YEAR = {1993},	PAGES = {251-276},
  DOI= {10.1145/169711.169704}
  }
  @inproceedings{hamilton2017inductive,
  title={Inductive representation learning on large graphs},
  author={Hamilton, William L and Ying, Rex and Leskovec, Jure},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={1025--1035},
  year={2017}
}

@inproceedings{Fey/Lenssen/2019,
  title={Fast Graph Representation Learning with {PyTorch Geometric}},
  author={Fey, Matthias and Lenssen, Jan E.},
  booktitle={ICLR Workshop on Representation Learning on Graphs and Manifolds},
  year={2019},
}
@article{van2008visualizing,
  title={Visualizing data using {t-SNE}},
  author={Van der Maaten, Laurens and Hinton, Geoffrey},
  journal={Journal of machine learning research},
  volume={9},
  number={11},
  year={2008}
}

@inproceedings{kipf2016semi,
  author    = {Thomas N. Kipf and
               Max Welling},
  title     = {Semi-Supervised Classification with Graph Convolutional Networks},
  booktitle = {5th International Conference on Learning Representations, {ICLR} 2017},
  year      = {2017}
}

@book{boyd2018introduction,
  title={Introduction to applied linear algebra: vectors, matrices, and least squares},
  author={Boyd, Stephen and Vandenberghe, Lieven},
  year={2018},
  publisher={Cambridge university press}
}

@incollection{kuhn2014nonlinear,
  title={Nonlinear programming},
  author={Kuhn, Harold W and Tucker, Albert W},
  booktitle={Traces and emergence of nonlinear programming},
  pages={247--258},
  year={2014},
  publisher={Springer}
}

@article{goodfellow2020generative,
  title={Generative adversarial networks},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
  journal={Communications of the ACM},
  volume={63},
  number={11},
  pages={139--144},
  year={2020},
  publisher={ACM New York, NY, USA}
}

@article{zhou2020towards,
  title={Towards deeper graph neural networks with differentiable group normalization},
  author={Zhou, Kaixiong and Huang, Xiao and Li, Yuening and Zha, Daochen and Chen, Rui and Hu, Xia},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={4917--4928},
  year={2020}
}

@inproceedings{velivckovic2017graph,
  author    = {Petar Velickovic and
               Guillem Cucurull and
               Arantxa Casanova and
               Adriana Romero and
               Pietro Li{\`{o}} and
               Yoshua Bengio},
  title     = {Graph Attention Networks},
  booktitle = {6th International Conference on Learning Representations, {ICLR} 2018},
  year      = {2018}
}

 @software{trimesh,
	author = {{Dawson-Haggerty et al.}},
	title = {Trimesh},
	url = {https://trimsh.org/},
	version = {3.2.0},
	date = {2019-12-8},
	year = {2019}
}

@inproceedings{qi2017pointnet,
  title={{PointNet}: Deep learning on point sets for {3D} classification and segmentation},
  author={Qi, Charles R and Su, Hao and Mo, Kaichun and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={652--660},
  year={2017}
}

@article{chang2015shapenet,
  title={{ShapeNet}: An information-rich {3D} model repository},
  author={Chang, Angel X and Funkhouser, Thomas and Guibas, Leonidas and Hanrahan, Pat and Huang, Qixing and Li, Zimo and Savarese, Silvio and Savva, Manolis and Song, Shuran and Su, Hao and others},
  journal={arXiv preprint arXiv:1512.03012},
  year={2015}
}

@BOOK (FolDamFeiHug.etal93,
	AUTHOR = {Foley, James D. and van Dam, Andries and
		Feiner, Stephen K. and Hughes, John F. and Phillips, R.},
	TITLE = {Introduction to Computer Graphics},
	PUBLISHER = {Addison-Wesley},
	YEAR = {1993} )

@ARTICLE{Kobbelt97-USHDR,
	author = {L. Kobbelt and M. Stamminger and H.-P. Seidel},
	title = {Using Subdivision on Hierarchical Data to Reconstruct Radiosity
		Distribution},
	JOURNAL = cgforum,
	volume = 16,	number = 3,	pages = {C347-C355},
	year = 1997,
	DOI = {10.1111/1467-8659.16.3conferenceissue.36},
	note = {(Proc. Eurographics'97)
	       \httpsAddr{//diglib.eg.org/handle/10.2312/8393}} }

@INPROCEEDINGS{Lafortune97-NARF,
	author = {Eric P. Lafortune and Sing-Choong Foo and Kenneth E. Torrance and
		Donald P. Greenberg},
	title = {Non-Linear Approximation of Reflectance Functions},
	booktitle = {Proc. SIGGRAPH '97},
	volume = 31,	pages = {117-126},
	year = 1997,
	DOI = {10.1145/258734.258801}
  }

@ARTICLE (Lous90,
	AUTHOR = {Y. Le Lous},
	TITLE = {Report on the {F}irst {E}urographics {W}orkshop on {V}isualization in
		{S}cientific {C}omputing},
	JOURNAL = cgforum,
	VOLUME = {9},	NUMBER = {4},
	MONTH = dec,	YEAR = {1990},	PAGES = {371-372},
  DOI= {10.1111/j.1467-8659.1990.tb00430.x}
  )

@ARTICLE (Seidel93,
	AUTHOR = {Seidel, Hans-Peter},
	TITLE = {Polar Forms for Geometrically Continuous Spline Curves of
		Arbitrary Degree},
	JOURNAL = tog,
	VOLUME = {12},	NUMBER = {1},
	MONTH = Jan,	YEAR = {1993},	PAGES = {1-34},
  DOI= {10.1145/169728.169726}
  )

@book{tapp2016differential,
  title={Differential geometry of curves and surfaces},
  author={Tapp, Kristopher},
  year={2016},
  publisher={Springer}
}

@article{huang2017topology,
  title={Topology-controlled reconstruction of multi-labelled domains from cross-sections},
  author={Huang, Zhiyang and Zou, Ming and Carr, Nathan and Ju, Tao},
  journal={ACM Transactions on Graphics (TOG)},
  volume={36},
  number={4},
  pages={1--12},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@article{zou2015topology,
  title={Topology-constrained surface reconstruction from cross-sections},
  author={Zou, Ming and Holloway, Michelle and Carr, Nathan and Ju, Tao},
  journal={ACM Transactions on Graphics (TOG)},
  volume={34},
  number={4},
  pages={1--10},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@article{lazar2018robust,
  title={Robust optimization for topological surface reconstruction},
  author={Lazar, Roee and Dym, Nadav and Kushinsky, Yam and Huang, Zhiyang and Ju, Tao and Lipman, Yaron},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={1--10},
  year={2018},
  publisher={ACM New York, NY, USA}
}
@article{sharma2017signed,
  title={Signed distance based {3D} surface reconstruction from unorganized planar cross-sections},
  author={Sharma, Ojaswa and Agarwal, Nidhi},
  journal={Computers \& Graphics},
  volume={62},
  pages={67--76},
  year={2017},
  publisher={Elsevier}
}


@article{amini2013geometric,
  title={Geometric tomography with topological guarantees},
  author={Amini, Omid and Boissonnat, Jean-Daniel and Memari, Pooran},
  journal={Discrete \& Computational Geometry},
  volume={50},
  number={4},
  pages={821--856},
  year={2013},
  publisher={Springer}
}


@article{bajaj1996arbitrary,
  title={Arbitrary topology shape reconstruction from planar cross sections},
  author={Bajaj, Chandrajit L and Coyle, Edward J and Lin, Kwun-Nan},
  journal={Graphical models and image processing},
  volume={58},
  number={6},
  pages={524--543},
  year={1996},
  publisher={Elsevier}
}


@inproceedings{hui2020progressive,
  title={Progressive point cloud deconvolution generation network},
  author={Hui, Le and Xu, Rui and Xie, Jin and Qian, Jianjun and Yang, Jian},
  booktitle={Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XV 16},
  pages={397--413},
  year={2020},
  organization={Springer}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}


@inproceedings{hertz2019pointgmm,
  title={{PointGMM}: a Neural {GMM} Network for Point Clouds},
  author={Hertz, Amir and Hanocka, Rana and Giryes, Raja and Cohen-Or, Daniel},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  year={2020}
}

@inproceedings{mandikal2019dense,
  title={Dense {3D} point cloud reconstruction using a deep pyramid network},
  author={Mandikal, Priyanka and Radhakrishnan, Venkatesh Babu},
  booktitle={2019 IEEE Winter Conference on Applications of Computer Vision (WACV)},
  pages={1052--1060},
  year={2019},
  organization={IEEE}
}

@inproceedings{fan2017point,
  title={A point set generation network for {3D} object reconstruction from a single image},
  author={Fan, Haoqiang and Su, Hao and Guibas, Leonidas J},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={605--613},
  year={2017}
}

@inproceedings{han2019multi,
  title={Multi-angle point {cloud-VAE}: Unsupervised feature learning for {3D} point clouds from multiple angles by joint self-reconstruction and half-to-half prediction},
  author={Han, Zhizhong and Wang, Xiyang and Liu, Yu-Shen and Zwicker, Matthias},
  booktitle={2019 IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={10441--10450},
  year={2019},
  organization={IEEE}
}


@inproceedings{wen2020point,
  title={Point cloud completion by skip-attention network with hierarchical folding},
  author={Wen, Xin and Li, Tianyang and Han, Zhizhong and Liu, Yu-Shen},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={1939--1948},
  year={2020}
}

@inproceedings{lin2018learning,
  title={Learning efficient point cloud generation for dense {3D} object reconstruction},
  author={Lin, Chen-Hsuan and Kong, Chen and Lucey, Simon},
  booktitle={proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  number={1},
  year={2018}
 }
 
 
 @article{HUANG2002149,
title = {Combinatorial manifold mesh reconstruction and optimization from unorganized points with arbitrary topology},
journal = {Computer-Aided Design},
volume = {34},
number = {2},
pages = {149-165},
year = {2002},
issn = {0010-4485},
author = {J Huang and C.H Menq},
keywords = {Shape recovery, Surface reconstruction, Mesh optimization, Curvature estimation},
}

@inproceedings{kanazawa2018learning,
  title={Learning category-specific mesh reconstruction from image collections},
  author={Kanazawa, Angjoo and Tulsiani, Shubham and Efros, Alexei A and Malik, Jitendra},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={371--386},
  year={2018}
}

@article{li2020online,
  title={Online adaptation for consistent mesh reconstruction in the wild},
  author={Li, Xueting and Liu, Sifei and De Mello, Shalini and Kim, Kihwan and Wang, Xiaolong and Yang, Ming-Hsuan and Kautz, Jan},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={15009--15019},
  year={2020}
}

@inproceedings{sarmad2019rl,
  title={{RL-GAN-Net}: A reinforcement learning agent controlled gan network for real-time point cloud shape completion},
  author={Sarmad, Muhammad and Lee, Hyunjoo Jenny and Kim, Young Min},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5898--5907},
  year={2019}
}


@inproceedings{pan2019deep,
  title={Deep mesh reconstruction from single {RGB} images via topology modification networks},
  author={Pan, Junyi and Han, Xiaoguang and Chen, Weikai and Tang, Jiapeng and Jia, Kui},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9964--9973},
  year={2019}
}



@inproceedings{boissonnat2007shape,
  title={Shape reconstruction from unorganized cross-sections},
  author={Boissonnat, Jean-Daniel and Memari, Pooran},
  booktitle={Symposium on geometry processing},
  pages={89--98},
  year={2007},
  organization={Citeseer}
}

@inproceedings{memari2008provably,
  title={Provably Good {2D} Shape Reconstruction from Unorganized Cross-Sections},
  author={Memari, Pooran and Boissonnat, Jean-Daniel},
  booktitle={Computer Graphics Forum},
  volume={27},
  number={5},
  pages={1403--1410},
  year={2008},
  organization={Wiley Online Library}
}


@inproceedings{liu2008surface,
  title={Surface reconstruction from non-parallel curve networks},
  author={Liu, Lu and Bajaj, Chandrajit and Deasy, Joseph O and Low, Daniel A and Ju, Tao},
  booktitle={Computer Graphics Forum},
  volume={27},
  number={2},
  pages={155--163},
  year={2008},
  organization={Wiley Online Library}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in neural information processing systems},
  pages={5998--6008},
  year={2017}
}

@InProceedings{Park_2019_CVPR_DEEPSDF,
author = {Park, Jeong Joon and Florence, Peter and Straub, Julian and Newcombe, Richard and Lovegrove, Steven},
title = {{DeepSDF}: Learning Continuous Signed Distance Functions for Shape Representation},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2019}
}


@article{bernardini1999ball,
  title={The ball-pivoting algorithm for surface reconstruction},
  author={Bernardini, Fausto and Mittleman, Joshua and Rushmeier, Holly and Silva, Cl{\'a}udio and Taubin, Gabriel},
  journal={IEEE transactions on visualization and computer graphics},
  volume={5},
  number={4},
  pages={349--359},
  year={1999},
  publisher={IEEE}
}

@article{huang2019variational,
  title={Variational implicit point set surfaces},
  author={Huang, Zhiyang and Carr, Nathan and Ju, Tao},
  journal={ACM Transactions on Graphics (TOG)},
  volume={38},
  number={4},
  pages={1--13},
  year={2019},
  publisher={ACM New York, NY, USA}
}


@inproceedings{kahzdan2006poisson,
title={Poisson Surface Reconstruction},
author={M. Kazhdan and M. Bolitho and H. Hoppe},
booktitle={Eurographics},
year={2006}

}


@inproceedings{atzmon2020sal,
  title={Sal: Sign agnostic learning of shapes from raw data},
  author={Atzmon, Matan and Lipman, Yaron},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2565--2574},
  year={2020}
}

@article{douglas1973algorithms,
  title={Algorithms for the reduction of the number of points required to represent a digitized line or its caricature},
  author={Douglas, David H and Peucker, Thomas K},
  journal={Cartographica: the international journal for geographic information and geovisualization},
  volume={10},
  number={2},
  pages={112--122},
  year={1973},
  publisher={University of Toronto Press}
}

@incollection{floater2006parameterization,
  title={Parameterization for curve interpolation},
  author={Floater, Michael S and Surazhsky, Tatiana},
  booktitle={Studies in Computational Mathematics},
  volume={12},
  pages={39--54},
  year={2006},
  publisher={Elsevier}
}


@article{Zhou2018_open3d,
    author    = {Qian-Yi Zhou and Jaesik Park and Vladlen Koltun},
    title     = {{Open3D}: {A} Modern Library for {3D} Data Processing},
    journal   = {arXiv:1801.09847},
    year      = {2018}
}

@misc{nlopt,
  author       = {"Steven G. Johnson"},
  title        = {The {NLopt} nonlinear-optimization package},
url = {"http://github.com/stevengj/nlopt"},
year = {2021}
}
@article{bermano2011online,
  title={Online reconstruction of {3D} objects from arbitrary cross-sections},
  author={Bermano, Amit and Vaxman, Amir and Gotsman, Craig},
  journal={ACM Transactions on Graphics (TOG)},
  volume={30},
  number={5},
  pages={1--11},
  year={2011},
  publisher={ACM New York, NY, USA}
}

@article{yin2018p2p,
  title={P2p-net: Bidirectional point displacement net for shape transform},
  author={Yin, Kangxue and Huang, Hui and Cohen-Or, Daniel and Zhang, Hao},
  journal={ACM Transactions on Graphics (TOG)},
  volume={37},
  number={4},
  pages={1--13},
  year={2018},
  publisher={ACM New York, NY, USA}
}
